Table2Vec: Neural Word and Entity Embeddings for Table Population and Retrieval

Tables contain valuable knowledge in a structured form. We employ neural language modeling approaches to embed tabular data into vector spaces. Specifically, we consider different table elements, such caption, column headings, and cells, for training word and entity embeddings. These embeddings are then utilized in three particular table-related tasks, row population, column population, and table retrieval, by incorporating them into existing retrieval models as additional semantic similarity signals. Evaluation results show that table embeddings can significantly improve upon the performance of state-of-the-art baselines.

==> other-inputs/fig-col-alpha.tex <==
\begin{figure}[t]
\centering
    \includegraphics[width = 0.4\textwidth]{cikm2019-table/figure/col-alpha.png}
    \caption{Effect of varying the interpolation parameters for combination method in column population.}
    \label{fig:col:alpha}
\end{figure} 
%

==> other-inputs/fig-eva-gt.tex <==
\begin{figure}[t]
\centering

    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width = \textwidth]{cikm2019-table/figure/row.png}
        \subcaption{Row population}
        \label{fig:gt:row}
    \end{subfigure}
    \hspace{0.5em}
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width = \textwidth]{cikm2019-table/figure/col.png}
        \subcaption{Column population}
        \label{fig:gt:col}        
    \end{subfigure}
    \hspace{0.5em}
    \caption{Illustration of evaluation methodology against table population. $E$ and $L$ represent the seed entities and seed labels respectively, and $gt$ is the corresponding ground truth.}
    \label{fig:eva:gt}
\end{figure} 
%

==> other-inputs/fig-fusion.tex <==
%
\begin{figure*}[t]
\centering
    \includegraphics[width = 0.8\textwidth]{cikm2019-table/figure/fusion.png}
    \caption{Illustration of computing query-table similarity using semantic representations.}
    \label{fig:fusion}
\end{figure*} 
%

==> other-inputs/fig-row-alpha.tex <==
%
\begin{figure}[t]
\centering
    \begin{subfigure}[b]{0.14\textwidth}
        \centering
        \includegraphics[width = \textwidth]{cikm2019-table/figure/BL1-alpha.png}
        \subcaption{BL1}
        \label{fig:bl1:alp}
    \end{subfigure}
    \hspace{0.5em}
    \begin{subfigure}[b]{0.14\textwidth}
        \centering
        \includegraphics[width = \textwidth]{cikm2019-table/figure/BL2-alpha.png}
        \subcaption{BL2}
        \label{fig:bl2:alp}        
    \end{subfigure}
    \hspace{0.5em}
    \begin{subfigure}[b]{0.14\textwidth}
        \centering
        \includegraphics[width = \textwidth]{cikm2019-table/figure/BL3-alpha.png}
        \subcaption{BL3}
        \label{fig:bl3:alp} 
    \end{subfigure}
    \hspace{0.5em}
    \caption{Effect of varying the interpolation parameters for combination methods in row population.}
    \label{fig:row:alpha}
\end{figure} 
%

==> other-inputs/fig-skip-gram.tex <==
\begin{figure}[t]
\centering
    \includegraphics[width = 0.35\textwidth]{cikm2019-table/figure/skip-gram.png}
    \caption{The skip-gram architecture.}
    \label{fig:skip}
\end{figure} 
%

==> other-inputs/fig-sub-qrl.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.4\textwidth]{cikm2019-table/figure/sub_query.png}
%	\vspace{-0.1in}
	\caption{Table retrieval results against query subsets in terms of NDCG@20.}
	\label{fig:sub:qry}
\end{figure}

==> other-inputs/tab-features.tex <==
\begin{table*}[t]
  \centering
  %\scriptsize
  \caption{Summery of features used for table retrieval task~\citep{Zhang:2018:AHT}.}
    \begin{tabular}{ l llc ll }
    \toprule
    \textbf {Feature Description} &  &\\
    \midrule
     $q_{len}$ & Sum of terms in the query $q$& \\
     $idf_{f}$ & Sum of query idf scores in the field f &\\
     numRows & Number of table rows &  \\
	 numCols &  Number of table columns &  \\
	 numEmptyCells & Number of empty tabular cells &\\
	 PMI & The Attribute Correlation Statistics Database based schema coherency score &\\
	 inLinks & Number of in-links to the page that contains the table &\\
	 outLinks & Number of out-links from the page that contains the table &\\
	 pageViews & Number of page views &\\
	 tableImportance & The inverse of number of tables on the page &\\
	 tablePageRatio & Ratio of table size to page size &\\
	 \#hitsLC & Total query term frequency in the leftmost column cells & \\
	 \#hitsSLC & Total query term frequency in second-to-leftmost column cells & \\
	 \#hitsB & Total query term frequency in the table data &\\
	 qInPgTitle & Ratio of number of query terms occurrences in page title to total number of terms & \\
	 qInTableTitle & Ratio of number of query terms occurrences in table title to total number of terms &\\
	 yRank & Rank of the table's Wikipedia page given by Web search engine for the query & \\
	 simInMLM & score given by Mixture Language Models between query and different table fields &\\
    \bottomrule
  \end{tabular}
  \label{tab:lsr}
\end{table*}
